UCSG-Net -- Unsupervised Discovering of Constructive Solid Geometry Tree

Signed distance field (SDF) is a prominent implicit representation of 3D meshes. Methods that are based on such representation achieved state-of-the-art 3D shape reconstruction quality. However, these methods struggle to reconstruct non-convex shapes. One remedy is to incorporate a constructive solid geometry framework (CSG) that represents a shape as a decomposition into primitives. It allows to embody a 3D shape of high complexity and non-convexity with a simple tree representation of Boolean operations. Nevertheless, existing approaches are supervised and require the entire CSG parse tree that is given upfront during the training process. On the contrary, we propose a model that extracts a CSG parse tree without any supervision - UCSG-Net. Our model predicts parameters of primitives and binarizes their SDF representation through differentiable indicator function. It is achieved jointly with discovering the structure of a Boolean operators tree. The model selects dynamically which operator combination over primitives leads to the reconstruction of high fidelity. We evaluate our method on 2D and 3D autoencoding tasks. We show that the predicted parse tree representation is interpretable and can be used in CAD software.

==> sections/limitations-feature-work.tex <==
\section{Limitations and future work}

Limitations:
\begin{itemize}
    \item Sensitive to the number of relation predictions layers
    \item Inductive biases to the high variance initialization
    \item Unclear how to properly threshold values
\end{itemize}
    
Future work:
\begin{itemize}
    \item Integration with BSP-Net and CvxNets. These approaches can approximate any convex shape that can be easily modified during learning (no inductive biases)
    \item More analytical shapes (knowledge encoding)
    \item Dynamic number of shapes
    \item Explanations are not parsimonous
    \item Only shapes taken to the relation are sampled but not the relation itself
    \item Application for geometrical problems such as medical data where one can approximate shapes of tissues using analytical equations
\end{itemize}
